Can Encrypted DNS Be Fast?

In this paper, we study the performance of encrypted DNS protocols and conventional DNS from thousands of home networks in the United States, over one month in 2020. We perform these measurements from the homes of 2,693 participating panelists in the Federal Communications Commission's (FCC) Measuring Broadband America program. We found that clients do not have to trade DNS performance for privacy. For certain resolvers, DoT was able to perform faster than DNS in median response times, even as latency increased. We also found significant variation in DoH performance across recursive resolvers. Based on these results, we recommend that DNS clients (e.g., web browsers) should periodically conduct simple latency and response time measurements to determine which protocol and resolver a client should use. No single DNS protocol nor resolver performed the best for all clients.

==> figures/tier_vs_latency.tex <==
\begin{figure*}[t!]
    \centering
    \subfigure[Resolver X]{%
        \includegraphics[width=0.31\textwidth]{figures/x_tier_v_latency}
        \label{fig:x_tier_v_latency}
    }
    \hfill
    \subfigure[Resolver Y]{%
        \includegraphics[width=0.31\textwidth]{figures/y_tier_v_latency}
        \label{fig:y_tier_v_latency}
    }
    \hfill
    \subfigure[Resolver Z]{%
        \includegraphics[width=0.31\textwidth]{figures/z_tier_v_latency}
        \label{fig:z_tier_v_latency}
    }
    \caption{Probability density functions for latencies to resolvers broken up by downstream throughput.}
    \label{fig:tier_v_latency}
\end{figure*}


==> sections/background.tex <==
\section{Background on DNS Privacy}\label{sec:background}
Before users can load a web page, their browser must \emph{resolve} a series of domain names (\eg, \texttt{nytimes.com}) into IP addresses of the servers that hold the content.
Each domain name is typically resolved in several steps.
First, users send a DNS request for a domain name to a \emph{recursive resolver}.
The recursive resolver is responsible for translating the domain name into an IP address on behalf of the user.
If the recursive resolver does not already know the answer (\ie, has it cached), it will issue queries to other DNS servers in the global DNS hierarchy.
This includes the root server, the top-level domain server that corresponds to a domain name (\eg, \texttt{.com} for \texttt{nytimes.com}), and finally the authoritative server for a given domain.

The original design of the DNS protocol does not include safeguards for privacy.
For example, conventional DNS traffic is not encrypted, so any eavesdropper sitting between a user and a recursive resolver can see what domain names the user is querying.
Given visibility into a user's DNS traffic, eavesdroppers can learn the browsing habits of users~\cite{zhu2015connection,rfc7626}.

In recent years, several protocols have been deployed encrypt DNS requests between DNS clients (\eg, browser users) and recursive resolvers.
For example, in 2016, Hu et al. introduced DNS-over-TLS (or ``DoT'')~\cite{zhu2015connection}.
DoT establishes a TLS session over port 853 between a client and a recursive resolver between any traffic is sent.
This enables users to encrypt their DNS requests, preventing eavesdroppers from inferring which websites they are visiting.
DoT has not seen widespread adoption in most operating systems, but it has been implemented on Android, which opportunistically establishes DoT connections to recursive resolvers when it's available~\cite{android-dot}.

In 2018, Hoffman et al. developed DNS-over-HTTPS~\cite{rfc8484}.
DoH is similar to DoT in that it encrypts DNS traffic between clients and recursive resolvers using TLS.
However, unlike DoT, DoH encodes requests and responses into the payload of HTTP packets, and all traffic is sent over port 443.
This enables clients to mix their DoH traffic with traditional HTTPS traffic, which is also sent over port 443.

In this paper, we do not investigate the privacy or anti-censorship properties offered by each protocol.
Rather, we are focused on comparing how DNS, DoT, and DoH perform across diverse networks and geographic regions.
We believe such measurements are necessary for users and browser vendors to make informed decisions about protocol choice for this crucial function of the Internet.


==> tables/coefficients.tex <==
\begin{table}[t]
    \centering
    \tiny
    \resizebox{\columnwidth}{!}{\begin{tabular}{l|rr|rr|rr}
        \toprule                                     & \multicolumn{2}{c|}{\textbf{DNS}}                   & \multicolumn{2}{c|}{\textbf{DoT}}  & \multicolumn{2}{c}{\textbf{DoH}}                        \\
        \textbf{Recursive resolver}                  & \multicolumn{1}{c}{\textbf{L}}                           & \multicolumn{1}{c|}{\textbf{T}}                       & \multicolumn{1}{c}{\textbf{L}}                & \multicolumn{1}{c|}{\textbf{T}}               & \multicolumn{1}{c}{\textbf{L}} & \multicolumn{1}{c}{\textbf{T}} \\
        \midrule
        Resolver X                                & 0.070                                      & -0.041                                     & 0.116                   & -0.041                   & 0.170   & -0.086     \\
        \rowcolor{Gray} Resolver Y& 0.080  & -0.042 & 0.068                   & -0.031                   & 0.097   & -0.049     \\
        Resolver Z                                & 0.079                                      & -0.041                                     & 0.080                   & -0.032                   & 0.116   & -0.037     \\
        \rowcolor{Gray}Default  & -0.012 & -0.029 & -                       & -                        & -       & -          \\
        \bottomrule
    \end{tabular}}
    \caption{Pearson correlation coefficients for latency (L) and downstream throughput (T) against DNS response times.}
    \label{tab:correlations}
\end{table}


==> tables/intro.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \begin{tabular}{|p{6cm}|c|c|}
        \hline
        Encrypted protocols add overhead in as they require TCP and TLS connection establishment. We observe up to 31.2 ms for TCP connection setup and 106.1 ms for TLS.  & \S\ref{sec:connection} &  Fig~\ref{fig:dot_doh_setup_times} \\ \hline
        There can be significant variation in performance between recursive resolvers. Median query response times changed by as much as 23.7 ms between two public DoH resolvers. & \S\ref{sec:dnstimesoverall} & Fig~\ref{fig:overall_dns_timings}\\\hline
        There is heterogeneity in DNS performance between ISPs. For one ISP, the median DoT response time for a public resolver was 11 ms faster than DNS. For another ISP, the median DoT response time for the same resolver was 30.7 ms slower than DNS. & \S\ref{sec:isp_comparison} & Fig~\ref{fig:isp_timings}\\\hline
        Latency to the resolver has a large effect, particularly for DoH. When the average latency to a public DoH resolver was greater than or equal to 50 ms, the median query response time was 100.1 ms. When the average latency to the same resolver was between 25 ms and 50 ms, the median query response time dropped to 59.8 ms. & \S\ref{sec:latencies} & Fig~\ref{fig:avg_latency_dns_timings}
        \\\hline
        Downstream throughput also affects DNS performance, particularly for DoH. When downstream throughput was less than 25 Mbps, the median query response time for a DoH resolver was 75.2 ms. When throughput was between 25 Mbps and 400 Mbps, the median query response time for the same resolver was 41.2 ms. & \S\ref{sec:bandwidth_results} & Fig~\ref{fig:package_down_dns_timings}
        \\\hline
        Latency has a higher correlation to DNS performance than downstream throughput. & \S\ref{sec:tiervlatency} & Fig~\ref{fig:tier_v_latency}
        \\\hline
    \end{tabular}
    \caption{Main results.}
    \label{tab:intro}
\end{table}


==> tables/isp_counts.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabularx}{0.7\linewidth}{Xr}
        \toprule
        \textbf{Internet Service Provider}
        & \textbf{Whiteboxes}
        \\
        \midrule
        ISP A
        & 201
        \\
        \rowcolor{Gray}
        ISP B
        & 202
        \\
        ISP C
        & 192
        \\
        \rowcolor{Gray}
        ISP D
        & 144
        \\
        ISP E
        & 141
        \\
        \bottomrule
    \end{tabularx}
    \caption{Number of Whiteboxes in each ISP.}
    \label{tab:isp_counts}
\end{table}


==> tables/package_down_counts.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabularx}{\columnwidth}{Xr}
        \toprule
        \textbf{Downstream ISP Throughput (Mbps)}
        & \textbf{Whiteboxes}
        \\
        \midrule
        (0, 25)
        & 849
        \\
        \rowcolor{Gray}
        {[}25, 400)
        & 1399
        \\
        {[}400, 800)
        & 355
        \\
        \rowcolor{Gray}
        {[}800, $\infty$)
        & 165
        \\
        \bottomrule
    \end{tabularx}
    \caption{Downstream ISP throughput packages used by whiteboxes.}
    \label{tab:package_down_counts}
\end{table}


==> tables/successful_measurement_counts.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabularx}{0.7\linewidth}{Xr}
        \toprule
        \textbf{Recursive resolver}
        & \textbf{Observations}
        \\
        \midrule
        Resolver X DNS
        & 467,552,206
        \\
        \rowcolor{Gray}
        Resolver X DoT
        & 464,857,763
        \\
        Resolver X DoH
        & 464,941,990
        \\
        \rowcolor{Gray}
        Resolver Y DNS
        & 493,481,882
        \\
        Resolver Y DoT
        & 465,385,639
        \\
        \rowcolor{Gray}
        Resolver Y DoH
        & 464,999,125
        \\
        Resolver Z DNS
        & 466,955,722
        \\
        \rowcolor{Gray}
        Resolver Z DoT
        & 464,718,474
        \\
        Resolver Z DoH
        & 463,079,872
        \\
        \rowcolor{Gray}
        Default DNS
        & 515,789,580
        \\
        \bottomrule
    \end{tabularx}
    \caption{Successful DNS measurements.}
    \label{tab:successful_measurement_counts}
\end{table}


==> tables/technology_counts.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabularx}{\linewidth}{ll}
        \toprule
        \textbf{Access Technology}
        & \textbf{Whiteboxes}
        \\
        \midrule
        DSL
        & 1071
        \\
        Cable
        & 881
        \\
        Fiber
        & 817
        \\
        Satellite
        & 26
        \\
        Unknown
        & 30
        \\
        \bottomrule
    \end{tabularx}
    \caption{Access technology usage.}
    \label{tab:technology_counts}
\end{table}

